Do the Findings of Document and Passage Retrieval Generalize to the Retrieval of Responses for Dialogues?

A number of learned sparse and dense retrieval approaches have recently been proposed and proven effective in tasks such as passage retrieval and document retrieval. In this paper we analyze with a replicability study if the lessons learned generalize to the retrieval of responses for dialogues, an important task for the increasingly popular field of conversational search. Unlike passage and document retrieval where documents are usually longer than queries, in response ranking for dialogues the queries (dialogue contexts) are often longer than the documents (responses). Additionally, dialogues have a particular structure, i.e. multiple utterances by different users. With these differences in mind, we here evaluate how generalizable the following major findings from previous works are: (F1) query expansion outperforms a no-expansion baseline; (F2) document expansion outperforms a no-expansion baseline; (F3) zero-shot dense retrieval underperforms sparse baselines; (F4) dense retrieval outperforms sparse baselines; (F5) hard negative sampling is better than random sampling for training dense models. Our experiments -- based on three different information-seeking dialogue datasets -- reveal that four out of five findings (F2-F5) generalize to our domain

==> tables/diff_lm_table.tex <==
\begin{table*}[]
% \small
\caption{Effectiveness of fine-tuned dense retrieval models when using different language models and intermediate training for each negative sampling procedures from Table~\ref{table:main_table_results}. Bold indicates the highest value within different negative sampling methods for the same setting. We observe the same phenomena of decreasing effectiveness for better negative sampling methods when using different language models and whether using intermediate training or not.}
\label{table:diff_lm_table}
\begin{tabular}{@{}llrrrrrrr@{}}
\toprule
 &  &  & \multicolumn{2}{c}{\textbf{\mantis{}}} & \multicolumn{2}{c}{\textbf{\msdialog{}}} & \multicolumn{2}{c}{\textbf{\ubuntu{}}} \\ \midrule
\textbf{Model} & \textbf{Intermediate data} & \textbf{Neg. Sampler} & \textbf{R@1} & \textbf{R@10} & \textbf{R@1} & \textbf{R@10} & \textbf{R@1} & \textbf{R@10} \\ \midrule
\multirow{6}{*}{Bi-encoder$_{mpnet-base}$} & \multirow{3}{*}{1.17B mul.sources} & Random (0) & \textbf{0.130} & \textbf{0.307} & \textbf{0.168} & \textbf{0.387} & \textbf{0.050} & \textbf{0.128} \\
 &  & \bm{} (1a) & 0.112 & 0.271 & 0.128 & 0.316 & 0.027 & 0.087 \\
 &  & Bi-encoder (3e) & 0.065 & 0.146 & 0.144 & 0.306 & 0.018 & 0.051 \\ \cmidrule(l){2-9} 
 & \multicolumn{1}{c}{\multirow{3}{*}{-}} & Random (0) & \textbf{0.070} & \textbf{0.172} & \textbf{0.114} & \textbf{0.308} & \textbf{0.021} & \textbf{0.063} \\
 & \multicolumn{1}{c}{} & \bm{} (1a) & 0.043 & 0.118 & 0.091 & 0.256 & 0.009 & 0.027 \\
 & \multicolumn{1}{c}{} & Bi-encoder (3e) & 0.032 & 0.087 & 0.083 & 0.205 & 0.002 & 0.019 \\ \midrule
\multirow{6}{*}{Bi-encoder$_{bert-base}$} & \multirow{3}{*}{500K \texttt{MSMarco-QA}} & Random (0) & \textbf{0.085} & \textbf{0.205} & \textbf{0.138} & \textbf{0.339} & \textbf{0.030} & \textbf{0.079} \\
 &  & \bm{} (1a) & 0.051 & 0.130 & 0.116 & 0.287 & 0.007 & 0.022 \\
 &  & Bi-encoder (3e) & 0.043 & 0.106 & 0.107 & 0.242 & 0.008 & 0.030 \\ \cmidrule(l){2-9} 
 & \multicolumn{1}{c}{\multirow{3}{*}{-}} & Random (0) & \textbf{0.029} & \textbf{0.092} & \textbf{0.063} & \textbf{0.200} & \textbf{0.012} & \textbf{0.038} \\
 & \multicolumn{1}{c}{} & \bm{} (1a) & 0.017 & 0.057 & 0.040 & 0.144 & 0.002 & 0.006 \\
 & \multicolumn{1}{c}{} & Bi-encoder (3e) & 0.011 & 0.041 & 0.034 & 0.119 & 0.000 & 0.009 \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/diff_loss_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\caption{Effectiveness of fine-tuned dense retrieval models when using different loss functions for each negative sampling procedures from Table~\ref{table:main_table_results}. We observe the same phenomena of decreasing effectiveness for better negative sampling methods with different loss functions. Bold indicates the highest value within different negative sampling methods for the same setting.}
\label{table:diff_loss}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
\textbf{} & \textbf{} & \multicolumn{2}{c}{\textbf{\mantis{}}} & \multicolumn{2}{c}{\textbf{\msdialog{}}} & \multicolumn{2}{c}{\textbf{\ubuntu{}}} \\ \midrule
\textbf{Loss} & \textbf{Negative Sampler} & \multicolumn{1}{l}{\textbf{R@1}} & \multicolumn{1}{l}{\textbf{R@10}} & \multicolumn{1}{l}{\textbf{R@1}} & \multicolumn{1}{l}{\textbf{R@10}} & \multicolumn{1}{l}{\textbf{R@1}} & \multicolumn{1}{l}{\textbf{R@10}} \\ \midrule
\multirow{3}{*}{MulNegRankLoss} & Random (0) & \textbf{0.130} & \textbf{0.307} & \textbf{0.168} & \textbf{0.387} & \textbf{0.050} & \textbf{0.128} \\
 & \bm{} (1a) & 0.112 & 0.271 & 0.128 & 0.316 & 0.027 & 0.087 \\
 & Bi-encoder (3e) & 0.065 & 0.146 & 0.144 & 0.306 & 0.018 & 0.051 \\ \midrule
\multirow{3}{*}{ContrastiveLoss} & Random (0) &  &  &  &  &  &  \\
 & \bm{} (1a) &  &  &  &  &  &  \\
 & Bi-encoder (3e) &  &  &  &  &  &  \\ \midrule
\multirow{3}{*}{TripletLoss} & Random (0) &  &  &  &  &  &  \\
 & \bm{} (1a) &  &  &  &  &  &  \\
 & Bi-encoder (3e) &  &  &  &  &  &  \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/evidence_for_h.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\caption{Summary of the findings of our follow-up experiments to explain why better negative samplers lead to worse dense retrieval results.}
\label{table:evidence_for_h}
\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{1}{l}{Experiment} & \multicolumn{1}{l}{Hypothesis} & \multicolumn{1}{l}{Evidence for H} \\ \midrule
E1 & \multirow{2}{*}{H1} & \cmark \\
E2 &  & \cmark \\ \midrule
E3 & \multirow{2}{*}{H2} & \xmark \\
E4 &  & \cmark \\ \midrule
E5 & \multirow{2}{*}{H3} &  \cmark \\
E6 &  & \xmark \\ \bottomrule
\end{tabular}
\end{table}

==> tables/hypothesis_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
% \small
\caption{Experiments to examine why better negatives sampling procedures lead to worse dense retrieval results. Bold indicates positive evidence for the corresponding hypothesis. We present the R@10 gains between the condition presented and the absence of the condition (4a--c on Table~\ref{table:main_table_results}) on E2--E5.}
\label{table:hypothesis_res}
\begin{tabular}{@{}llccc@{}}
\toprule
\multicolumn{5}{c}{E1} \\ \midrule
NS & Count & \mantis{} & \msdialog{} & \ubuntu{} \\ \midrule
Random (0) & \multirow{2}{*}{false $r^{-}$} & 0 & 0 & 0 \\
\bm{} (1a) &  & 0 & \textbf{4} & \textbf{2} \\
Bi-encoder (3e) &  & \textbf{11} & \textbf{4} & \textbf{15} \\ \midrule
\multicolumn{5}{c}{E2} \\ \midrule
 &  & \mantis{} & \msdialog{} & \ubuntu{} \\ \midrule
NS & Condition & R@10$\Delta$ & R@10$\Delta$ & R@10$\Delta$ \\ \midrule
\bm{} (1a) & \multirow{2}{*}{denoising} & -0.014 & \textbf{+0.042} & \textbf{+0.034} \\
Bi-encoder (3e) &  & \textbf{+0.170} & \textbf{+0.091} & \textbf{+0.056} \\ \midrule
\multicolumn{5}{c}{E3} \\ \midrule
 &  & \mantis{} & \msdialog{} & \ubuntu{} \\ \midrule
NS & Condition & R@10$\Delta$ & R@10$\Delta$ & R@10$\Delta$ \\ \midrule
\bm{} (1a) & \multirow{2}{*}{$r^{-}$ subset of $\set{U}$} & \textbf{-0.032} & +0.015 & \textbf{-0.010} \\
Bi-encoder (3e) &  & +0.034 & \textbf{-0.040} & \textbf{-0.003} \\ \midrule
\multicolumn{5}{c}{E4} \\ \midrule
 &  & \mantis{} & \msdialog{} & \ubuntu{} \\ \midrule
NS & Condition & R@10$\Delta$ & R@10$\Delta$ & R@10$\Delta$ \\ \midrule
\bm{} (1a) & \multirow{2}{*}{U$_{lu}$ as query} & -0.002 & \textbf{+0.044} & -0.008 \\
Bi-encoder (3e) &  & \textbf{+0.173} & \textbf{+0.042} & \textbf{+0.047} \\ \midrule
\multicolumn{5}{c}{E5} \\ \midrule
 &  & \mantis{} & \msdialog{} & \ubuntu{} \\ \midrule
NS & Corpus & R@10$\Delta$ & R@10$\Delta$ & R@10$\Delta$ \\ \midrule
\bm{} (1a) & \multirow{2}{*}{expanded} & -0.014 & \textbf{+0.031} & \textbf{+0.023} \\
Bi-encoder (3e) & & \textbf{+0.113} & \textbf{+0.028} & \textbf{+0.057}   \\ \midrule
\multicolumn{5}{c}{E6} \\ \midrule
 &  & \mantis{} & \msdialog{} & \ubuntu{} \\ \midrule
\multicolumn{2}{l}{NS} & R@10 & R@10 & R@10 \\ \midrule
\multicolumn{2}{l}{Random (0)} & 0.307 & 0.387 & 0.128 \\
\multicolumn{2}{l}{GenNegatives$_{Blenderbot}$} & 0.267 & 0.348 & \textbf{0.134} \\
\multicolumn{2}{l}{GenNegatives$_{DialoGPT}$} & 0.260 & 0.363 & 0.123 \\ \bottomrule
\end{tabular}
\end{table}
